Gromov-Wasserstein-like Distances in the Gaussian Mixture Models Space

The Gromov-Wasserstein (GW) distance is frequently used in machine learning to compare distributions across distinct metric spaces. Despite its utility, it remains computationally intensive, especially for large-scale problems. Recently, a novel Wasserstein distance specifically tailored for Gaussian mixture models (GMMs) and known as MW2 (mixture Wasserstein) has been introduced by several authors. In scenarios where data exhibit clustering, this approach simplifies to a small-scale discrete optimal transport problem, which complexity depends solely on the number of Gaussian components in the GMMs. This paper aims to incorporate invariance properties into MW2. This is done by introducing new Gromov-type distances, designed to be isometry-invariant in Euclidean spaces and applicable for comparing GMMs across different dimensional spaces. Our first contribution is the Mixture Gromov Wasserstein distance (MGW2), which can be viewed as a "Gromovized" version of MW2. This new distance has a straightforward discrete formulation, making it highly efficient for estimating distances between GMMs in practical applications. To facilitate the derivation of a transport plan between GMMs, we present a second distance, the Embedded Wasserstein distance (EW2). This distance turns out to be closely related to several recent alternatives to Gromov-Wasserstein. We show that EW2 can be adapted to derive a distance as well as optimal transportation plans between GMMs. We demonstrate the efficiency of these newly proposed distances on medium to large-scale problems, including shape matching and hyperspectral image color transfer.

==> rebuttal.tex <==
Comments :

Weakness:

    The innovation of this paper may be lacking. Can you highlight the difficulty in your proof?

    Although the algorithms in this paper are primarily designed for large-scale problems, I am still uncertain about their performance on smaller-scale problems. Since the paper focuses on large-scale settings, even if the performance on smaller scales is not good, it does not affect my overall opinion of the paper.


I advise the authors to divide the section 'Discussion' into conclusion and future work.

-------------
Answers :
Thank you for your review and your comments.  If you find the following answers satisfactory, we suggest including them in the article for greater clarity.

1. About the paper innovation: Gromov-Wasserstein distances are known to be computationally costly. If there have been attempts to reduce this computational burden by using more compact representations of the data (for instance with quantized GW, or entropic regularization of GW), to the best of our knowledge there is no approach in the literature leveraging the underlying structure of the data points to compute GW. GMM are widely used in machine learning and applied statistics (either directly on data or on features from data) and our goal was to study how GW could be made appropriate to compare directly such representations. This permits to reduce the computational complexity of GW from a large scale problem to a small scale depending only on the number of components in the chosen representations. The experiments show that even on large scale problems classicaly used in the literature, very simple GMM representations with only a few dozens of components give excellent results. 

About the difficulties: Although the definition of MGW is simply GW between two discrete distributions on the space of Gaussian measures and thus establishing its pseudometric properties doesn't present any major technical difficulty, there remains a few theoretical subtleties. Notably, on what condition do we have $ MGW_2(\mu,\nu) = 0 $? (see Section 3.1) Another difficulty which motivates the introduction of $ EW_2 $ in Section 4 is that it is not straightforward to obtain a transportation plan $ \pi $ between the points using $ MGW $.  

2. We believe our method is not adapted for small scale problems as computing GMMs is not useful in that case, and the GW problem can be solved directly.

3. Thank you for you suggestion about the section "Discussion". This has been taken into account in  the revised version.




---------------------------------


(X) One of the critical goals of this work seems to be having an invariant distance (to certain transformations) between probability measures; how the abstract and the introduction are written makes it sound like a nice byproduct. Consider rewriting to emphasize the fact that you aimed for invariance.

-> Thank you for this observation, we modified a few sentences both in the abstract and introduction to clarify this.

(X) In the abstract, introduce the abbreviation GMMs (currently, it is used but not introduced).

-> Done

(X) The title has a grammatical mistake it should be Wasserstein (note the s before the t) instead of Wassertein.

(X) P2 First line: footnotes should go after punctuation. 

(X) P2 Change: "is invariant to important families of transformations" to "is invariant to a given family of transformations''

(X) P3 Notations: I would call this section Notation (without the s); the same goes for the first line of this section.

(X) P3 and P4 This is mostly personal preference, but consider changing the format of the notation section to a couple of paragraphs inline instead of a list. The list occupies too much space and does not match the style of the rest of the paper.

(X) P5 Add a reference for the fact that $MW_2$ defines a metric on $GGM_\infty(R^d)$.

(X) P8 Before Proposition 2: 'developped' -> developed.

(X) The P8 Question before Proposition 3 is hard to parse; consider rewriting.

-> This sentence has been clarified.

(X) P8 The Euclidian norm is only one; it is defined in any dimension, but only one. Change the statement to say it is an isometry for the Euclidian norm.

(X) P8 Consider adding an Example environment for the example at the end of this page.

(X)P9 is hard to follow for the uninitiated; consider rewriting. Explicitly introduce $\pi*$ and $\omega*$. Don't call a matrix $Id$ if it is not the identity. Consider dropping the notation $A^{[d', d]}$ and simply write it explicitly in the definition of $T_{GGW_2}^{k, l}$.

(X) All of Page 9 feels unnecessary; it could be compressed to a paragraph at best. The authors are explaining how not to do things, which feels distracting.

-> The paragraph "difficulty of designing a transport plan" has been rewritten in a more compact way. 

(X) Page 11 Section 4: "explicit'' is NOT a verb but an adjective or noun.

(X) Page 11 Drop the use of "any'' in the sentence "we will suppose without any loss of generality that...'' (it's redundant).

(X) Page 13 Problems involving the Stiefel Manifold can often be solved via Riemannian optimization methods; consider trying https://www.manopt.org/, see https://www.nicolasboumal.net/book/IntroOptimManifolds_Boumal_2022.pdf for a reference.

-> You are right, we added the second reference in the paper.

(X) Page 14 What is the function $\kappa$ in the definition of $P^{{1}}$?

-> $ \kappa $ is the projection mapping on the Stiefel manifold, as explained at the beginning of 4.2.1


(X) Page 15 Use \colon (the command) as supposed to ":'' when defining functions.

(X) Page 17 Figure 5 is impossible to parse. Are you somehow comparing the error between the two methods? It seems that you are just plotting labels.

-> Figure 5 shows an embedding of the horse sequence in two dimensions. More precisely, we apply a multi-scale scaling (MDS) to the 45 x 45 matrix of pairwise distances between all 45 horse meshes. We do that both for MGW2 and MEW2. The output of the MDS is a set of 45 2D points. The interesting part here is that these 2D points are positioned in a circular fashion, which means that the distances seem to respect the periodic aspect of the sequence. This has been clarified in the text.



For the experiments, use a color-blind-friendly palette.

--> This will be modified upon acceptance of the paper. 

-------
More clearly state the advantages of MGW (and MEW) over qGW. 



--> Thank you for your review and your comments. About the comparison between MGW and qGW, first note that the MGW method primarly provides a distance between clouds of points before providing an heuristic coupling between them. This is not the case of the qGW method that directly derives an heuristic coupling which can then be reinjected in the objective function to derive a distance. Consequently to this difference of design between the two methods, MGW seems to be a more adequate choice than qGW for tasks that only require to assess a distance between clouds of points (see Figure 7) 
whereas qGW seems a more adequate choice for tasks that require a coupling between points. Still, we have shown in our experiments that the MGW method can also provide couplings, with performance equivalent to qGW in terms of accuracy despite being significantly slower in the small-to-medium scale setting of Table 1. Yet, we believe that an advantage of MGW over qGW for deriving couplings 
is that the MGW method decorrelates the number of clusters needed to achieve good accuracy from the number of points, which might be an interessing feature in larger scale settings.  


